Arrows of Math Reasoning Data Synthesis for Large Language Models: Diversity, Complexity and Correctness

Enhancing the mathematical reasoning of large language models (LLMs) demands high-quality training data, yet conventional methods face critical challenges in scalability, cost, and data reliability. To address these limitations, we propose a novel program-assisted synthesis framework that systematically generates a high-quality mathematical corpus with guaranteed diversity, complexity, and correctness. This framework integrates mathematical knowledge systems and domain-specific tools to create executable programs. These programs are then translated into natural language problem-solution pairs and vetted by a bilateral validation mechanism that verifies solution correctness against program outputs and ensures program-problem consistency. We have generated 12.3 million such problem-solving triples. Experiments demonstrate that models fine-tuned on our data significantly improve their inference capabilities, achieving state-of-the-art performance on several benchmark datasets and showcasing the effectiveness of our synthesis approach.

==> sec9-app.tex <==

\section{Implementation Details}



\section{Finetuning Details} \label{sec: Finetuning Details}

We finetune all models using LLaMA Factory []. Following previous work [], we set the learning rate to $2\times 10^{-5}$ and used the first 50 steps as warm-up steps with a cosine weight scheduler. All models were optimized using LoRA and AdamW on 8 NVIDIA A100 GPUs with a batch size of 64 (\ie a batch size of 8 per GPU).



\section{Mathematical Knowledge System}\label{app:system}


\begin{table}
  \centering
  \begin{tabular}{lc}
    \hline
    \textbf{Command} & \textbf{Output} \\
    \hline
    \verb|{\"a}|     & {\"a}           \\
    \verb|{\^e}|     & {\^e}           \\
    \verb|{\`i}|     & {\`i}           \\
    \verb|{\.I}|     & {\.I}           \\
    \verb|{\o}|      & {\o}            \\
    \verb|{\'u}|     & {\'u}           \\
    \verb|{\aa}|     & {\aa}           \\\hline
  \end{tabular}
  \begin{tabular}{lc}
    \hline
    \textbf{Command} & \textbf{Output} \\
    \hline
    \verb|{\c c}|    & {\c c}          \\
    \verb|{\u g}|    & {\u g}          \\
    \verb|{\l}|      & {\l}            \\
    \verb|{\~n}|     & {\~n}           \\
    \verb|{\H o}|    & {\H o}          \\
    \verb|{\v r}|    & {\v r}          \\
    \verb|{\ss}|     & {\ss}           \\
    \hline
  \end{tabular}
  \caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
  \label{tab:accents}
\end{table}




\section{Case Study}



\section{Prompts}

\subsection{Prompts for Mathematical Knowledge System Construction}


\subsection{Prompts for Program Mutation}

\lstset{
    basicstyle=\small\ttfamily, %
    breaklines=true, %
    columns=flexible, %
    showstringspaces=false, %
    breakindent=0pt,
}


\begin{table*}[t]
\centering
\caption{A Large Table Spanning Both Columns with a Single Column for Prompt}
\label{tab:large_table}
\begin{tabular}{p{0.9\textwidth}}
\toprule
\begin{lstlisting}
## Task Description
You are a mathematics professor skilled in programming. Given a Python program that describes the solution process of a math problem, your task is to rewrite the Python program to make the solution process and the solution goal more complex.

## Characteristics of the Given Python Program
1. The program primarily uses SymPy's symbolic computation capabilities to solve the math problem.
2. The last line of the program is a `print` statement that outputs the final solution.
3. The problem primarily tests the following knowledge points: {exer_kc_list}, where the format is <Grade-Unit-KnowledgePoint>.

## List of Rewriting Strategies
Rewriting methods include, but are not limited to:
- **Sub-function Calls**: Use the current SymPy functions as sub-functions to create new problems.
- **Intermediate Steps**: Treat the current solution goal as an intermediate result (i.e., a sub-problem) and create new variables as the final solution goal (i.e., a new problem).
- **Constraint Operations**:
  1. Add new constraints to make the solution process more complex (e.g., add boundary conditions).
  2. Modify existing constraints to make them more complex (e.g., change initial conditions).
- **Variable Operations**:
  1. Modify the coefficients of variables to increase difficulty (e.g., change small numbers to large numbers, integers to fractions, constants to variables, add exponents).
  2. Replace variables to increase difficulty (e.g., replace a single variable with multiple variables).
  3. Introduce new variables to increase the complexity of the final `print` statement output.
- **Constant Operations**:
  1. Modify constant values to increase difficulty (e.g., change small numbers to large numbers, integers to fractions, constants to variables, add exponents).
  2. Change constants to be controlled by multiple variables (e.g., add additional equations where the solutions are constants).
- **Expression Operations**:
  1. Introduce new terms to increase difficulty (e.g., add multiple terms).
  2. Modify expressions to make them more complex (e.g., convert expressions to fractions).
- **Code Segment Operations**:
  1. Add new code segments, such as conditional statements, variable increments, and loops, to make the solution process more complex.
  2. Replace current code segments to make the solution logic more complex.
- **SymPy API Operations**:
  1. Add new SymPy APIs to make the solution process more complex.
  2. Replace with more complex SymPy APIs.
  3. Relevant SymPy APIs for the knowledge points {exer_kc_list} are as follows:
  ```
  {kc2api_str}
  ```

## Output Format
The output should be in JSON format, and all generated programs should be summarized in the specified format, wrapped in "```rewrite_program_list ```". Each element in the list is a dictionary:
- The `program` field contains the rewritten program.
- The `methods` field is a dictionary where each key-value pair describes the rewriting method used.
- The `comment` field describes the number of times each rewriting method was used.

## Instructions
Please take the following SymPy program as the initial solution and generate {n_programs} rewritten versions, following the output format and adhering to the guidelines.
```
{exer_program}
```
\end{lstlisting} \\
\bottomrule
\end{tabular}
\end{table*}

\subsection{Prompts for Natural Language Reasoning Data Synthesis}


\subsection{Prompts for Natural Language Reasoning Data Correction Validation}



